Optimal Mean Estimation without a Variance

We study the problem of heavy-tailed mean estimation in settings where the variance of the data-generating distribution does not exist. Concretely, given a sample $\mathbf{X} = \{X_i\}_{i = 1}^n$ from a distribution $\mathcal{D}$ over $\mathbb{R}^d$ with mean $\mu$ which satisfies the following \emph{weak-moment} assumption for some ${\alpha \in [0, 1]}$: \begin{equation*} \forall \|v\| = 1: \mathbb{E}_{X \thicksim \mathcal{D}}[\lvert \langle X - \mu, v\rangle \rvert^{1 + \alpha}] \leq 1, \end{equation*} and given a target failure probability, $\delta$, our goal is to design an estimator which attains the smallest possible confidence interval as a function of $n,d,\delta$. For the specific case of $\alpha = 1$, foundational work of Lugosi and Mendelson exhibits an estimator achieving subgaussian confidence intervals, and subsequent work has led to computationally efficient versions of this estimator. Here, we study the case of general $\alpha$, and establish the following information-theoretic lower bound on the optimal attainable confidence interval: \begin{equation*} \Omega \left(\sqrt{\frac{d}{n}} + \left(\frac{d}{n}\right)^{\frac{\alpha}{(1 + \alpha)}} + \left(\frac{\log 1 / \delta}{n}\right)^{\frac{\alpha}{(1 + \alpha)}}\right). \end{equation*} Moreover, we devise a computationally-efficient estimator which achieves this lower bound.

==> content/glossary.tex <==
\usepackage{amsmath,amsthm,amssymb}
\usepackage{textcomp}
\usepackage{mathtools,bbm,xspace}
\usepackage{mathrsfs}
\usepackage{nicefrac}

\usepackage{ifxetex}

\usepackage[dvipsnames]{xcolor}
\usepackage{hyperref}
\RequirePackage[colorlinks,citecolor=blue,urlcolor=blue]{hyperref}
\RequirePackage[numbers]{natbib}

\usepackage[capitalise,nameinlink]{cleveref}
\crefname{lemma}{Lemma}{Lemmas}
\crefname{fact}{Fact}{Facts}
\crefname{theorem}{Theorem}{Theorems}
\crefname{corollary}{Corollary}{Corollaries}
\crefname{claim}{Claim}{Claims}
\crefname{example}{Example}{Examples}
\crefname{problem}{Problem}{Problems}
\crefname{remark}{Remark}{Remarks}
\crefname{definition}{Definition}{Definitions}
\crefname{assumption}{Assumption}{Assumptions}
\crefname{subsection}{Subsection}{Subsections}
\crefname{section}{Section}{Sections}

% \crefname{ALC@unique}{Line}{Lines}

\usepackage{ulem}
\usepackage{tcolorbox}
\usepackage{enumerate}
\usepackage{csquotes}
\usepackage{algorithm}
\usepackage{algorithmic}
\usepackage{tabularx}

\usepackage{bm}
\allowdisplaybreaks

\newtheorem{theorem}{Theorem}[section]
\newtheorem*{theorem*}{Theorem}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem*{lemma*}{Lemma}

\theoremstyle{definition}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{problem}[theorem]{Problem}
\newtheorem{assumption}[theorem]{Assumption}

\newtheorem{remark}[theorem]{Remark}
\newtheorem*{remark*}{Remark}

\newcommand\numberthis{\addtocounter{equation}{1}\tag{\theequation}}

% Norm Stuff
\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator*{\Tr}{\bm{Tr}}
\DeclareMathOperator*{\sgn}{sgn}

\DeclarePairedDelimiterX{\norm}[1]{\lVert}{\rVert}{#1}

\newcommand{\onenorm}[1]{\norm{#1}_1}
\newcommand{\twonorm}[1]{\norm{#1}_2}
\newcommand{\infnorm}[1]{\norm{#1}_\infty}
\newcommand{\trnorm}[1]{\norm{#1}_{\ast}}

\DeclarePairedDelimiterX{\abs}[1]{\lvert}{\rvert}{#1}
\DeclarePairedDelimiterX{\inp}[2]{\langle}{\rangle}{#1, #2}
\DeclarePairedDelimiter{\ceil}{\lceil}{\rceil}
\DeclarePairedDelimiter{\floor}{\lfloor}{\rfloor}
\DeclarePairedDelimiterX{\infdivx}[2]{(}{)}{%
  #1\;\delimsize\|\;#2%
}
\DeclareMathOperator*{\sign}{sign}

\newcommand{\mc}[1]{\mathcal{#1}}
\newcommand{\mb}[1]{\mathbb{#1}}

\newcommand{\sym}[1][n]{\mathbb{S}^{#1}}
\newcommand{\psd}[1][n]{\mathbb{S}_+^{#1}}
\newcommand{\lprp}[1]{\left(#1\right)}
\newcommand{\lbrb}[1]{\left\{#1\right\}}
\newcommand{\lsrs}[1]{\left[#1\right]}

% miscellaneous shortcuts
\newcommand{\Ind}{\boldsymbol{1}}
\newcommand{\SORT}{\mathsf{SORT}}
\newcommand{\supp}{\mathrm{supp}}
\newcommand{\Id}{\mathrm{Id}}
\newcommand{\bone}{\Ind}
\newcommand{\spec}{\mathsf{spec}}
\newcommand{\grad}{\nabla}

%special macros
\newcommand{\hu}{\hat{\mu}}


% better looking epsilon
\newcommand{\eps}{\varepsilon}
\newcommand{\vphi}{\varphi}

\newcommand{\svd}{\mathsf{SVDE}}
\newcommand{\distinct}{\mathrm{distinct} }
\newcommand{\calA}{\mathcal A}
\newcommand{\calB}{\mathcal B}
\newcommand{\calC}{\mathcal C}
\newcommand{\calD}{\mathcal D}
\newcommand{\calE}{\mathcal E}
\newcommand{\calF}{\mathcal F}
\newcommand{\calG}{\mathcal G}
\newcommand{\calH}{\mathcal H}
\newcommand{\calI}{\mathcal I}
\newcommand{\calJ}{\mathcal J}
\newcommand{\calK}{\mathcal K}
\newcommand{\calL}{\mathcal L}
\newcommand{\calM}{\mathcal M}
\newcommand{\calN}{\mathcal N}
\newcommand{\calO}{\mathcal O}
\newcommand{\calP}{\mathcal P}
\newcommand{\calQ}{\mathcal Q}
\newcommand{\calR}{\mathcal R}
\newcommand{\calS}{\mathcal S}
\newcommand{\calT}{\mathcal T}
\newcommand{\calU}{\mathcal U}
\newcommand{\calV}{\mathcal V}
\newcommand{\calW}{\mathcal W}
\newcommand{\calX}{\mathcal X}
\newcommand{\calY}{\mathcal Y}
\newcommand{\calZ}{\mathcal Z}

\newcommand{\cG}{\calG}

\newcommand{\bbB}{\mathbb B}
\newcommand{\bbS}{\mathbb S}
\newcommand{\bbR}{\mathbb R}
\newcommand{\bbZ}{\mathbb Z}
\newcommand{\bbI}{\mathbb I}
\newcommand{\bbQ}{\mathbb Q}
\newcommand{\bbP}{\mathbb P}
\newcommand{\bbE}{\mathbb E}

\newcommand{\R}{\bbR}


\newcommand{\bbeta}{\boldsymbol{\beta}}
\newcommand{\bdelta}{\boldsymbol{\delta}}
\newcommand{\bepsilon}{\boldsymbol{\epsilon}}
\newcommand{\blambda}{\boldsymbol{\lambda}}
\newcommand{\bomega}{\boldsymbol{\omega}}
\newcommand{\bpi}{\boldsymbol{\pi}}
\newcommand{\bnu}{\boldsymbol{\nu}}
\newcommand{\bphi}{\boldsymbol{\phi}}
\newcommand{\bvphi}{\boldsymbol{\varphi}}
\newcommand{\bpsi}{\boldsymbol{\psi}}
\newcommand{\brho}{\boldsymbol{\rho}}
\newcommand{\bsigma}{\boldsymbol{\sigma}}
\newcommand{\btau}{{\boldsymbol{\tau}}}
\newcommand{\btheta}{\boldsymbol{\theta}}
\newcommand{\bzeta}{\boldsymbol{\zeta}}
\newcommand{\ba}{\boldsymbol{a}}
\newcommand{\bb}{\boldsymbol{b}}
\newcommand{\bc}{\boldsymbol{c}}
\newcommand{\bd}{\boldsymbol{d}}
\newcommand{\be}{\boldsymbol{e}}
\newcommand{\boldf}{\boldsymbol{f}}
\newcommand{\bg}{\boldsymbol{g}}
\newcommand{\bh}{\boldsymbol{h}}
\newcommand{\bi}{\boldsymbol{i}}
\newcommand{\bj}{\boldsymbol{j}}
\newcommand{\bk}{\boldsymbol{k}}
\newcommand{\bell}{\boldsymbol{\ell}}
\newcommand{\bp}{\boldsymbol{p}}
\newcommand{\bq}{\boldsymbol{q}}
\newcommand{\br}{\boldsymbol{r}}
\newcommand{\bs}{\boldsymbol{s}}
% \newcommand{\bt}{\boldsymbol{t}}
\newcommand{\bu}{\boldsymbol{u}}
\newcommand{\bv}{\boldsymbol{v}}
\newcommand{\bw}{\boldsymbol{w}}
\newcommand{\bx}{{\boldsymbol{x}}}
\newcommand{\by}{\boldsymbol{y}}
\newcommand{\bz}{\boldsymbol{z}}
\newcommand{\bA}{\boldsymbol{A}}
\newcommand{\bB}{\boldsymbol{B}}
\newcommand{\bC}{\boldsymbol{C}}
\newcommand{\bD}{\boldsymbol{D}}
\newcommand{\bE}{\boldsymbol{E}}
\newcommand{\bF}{\boldsymbol{F}}
\newcommand{\bG}{\boldsymbol{G}}
\newcommand{\bH}{\boldsymbol{H}}
\newcommand{\bI}{\boldsymbol{I}}
\newcommand{\bJ}{\boldsymbol{J}}
\newcommand{\bL}{\boldsymbol{L}}
\newcommand{\bM}{\boldsymbol{M}}
\newcommand{\bP}{\boldsymbol{P}}
\newcommand{\bQ}{\boldsymbol{Q}}
\newcommand{\bR}{\boldsymbol{R}}
\newcommand{\bS}{\boldsymbol{S}}
\newcommand{\bT}{\boldsymbol{T}}
\newcommand{\bU}{\boldsymbol{U}}
\newcommand{\bV}{\boldsymbol{V}}
\newcommand{\bW}{\boldsymbol{W}}
\newcommand{\bX}{\boldsymbol{X}}
\newcommand{\bY}{\boldsymbol{Y}}
\newcommand{\bZ}{\boldsymbol{Z}}

\newcommand{\barw}{\bar{w}}


\renewcommand{\le}{\leqslant}
\renewcommand{\leq}{\leqslant}
\renewcommand{\ge}{\geqslant}
\renewcommand{\geq}{\geqslant}

\newcommand{\psdge}{\succcurlyeq}
\newcommand{\psdg}{\succ}
\newcommand{\psdle}{\preccurlyeq}
\newcommand{\psdl}{\prec}

\renewcommand{\emph}{\textit}
\newcommand{\rv}[1]{\boldsymbol{#1}}

\newcommand{\la}{\langle}
\newcommand{\ra}{\rangle}
\newcommand{\wt}[1]{\widetilde{#1}}
\newcommand{\wh}[1]{\widehat{#1}}
\newcommand{\wb}[1]{\widebar{#1}}

\usepackage{subcaption} 
\newcommand{\ignore}[1]{{\begin{comment}#1\end{comment}}}


% complexity classes

\def \poly {\text{poly}}
\def \RP {{\sf RP}}
\def \BPP {{\sf BPP}}
\def \NC {{\sf NC}}
\def \NE {{\sf NE}}
% \def \E {{\sf E}}
\def \poly { \text{\rm poly} }
\def \TC {{\sf TC}}
\def \DTS {{\sf DTS}}
% \def \R {{\cal R}}
\def \Z {{\mathbb Z}}
\def \majority {{\sf Majority}}
\def \P {{\sf P}}
\def \MA {{\sf MA}}
\def \A {{\sf A}}
\def \NP {{\sf NP}}
\def \EXP {{\sf EXP}}
\def \NTISP {{\sf NTISP}}
\def \DTISP {{\sf DTISP}}
\def \TISP {{\sf TISP}}
\def \TIME {{\sf TIME}}
\def \T {{\sf T}}
\def \Sig[#1] {{\sf \Sigma}_{#1} }
\def \Pie[#1] {{\sf \Pi}_{#1} }
\def \NTS {{\sf NTS}}
\def \NSP {{\sf NSPACE}}
\def \NSPACE {{\sf NSPACE}}
\def \BPACC {{\sf BPACC}}
\def \PH {{\sf PH}}
\def \ACC {{\sf ACC}}
\def \ASP {{\sf ASPACE}}
\def \M {{\sf M}}
\def \io {\textrm{\it i.o.-}}
\def \ATISP {{\sf ATISP}}
\def \SIZE {{\sf SIZE}}
\def \ioSIZE {{\sf ioSIZE}}
\def \PSIZE {{\sf PSIZE}}
\def \AT {{\sf ATIME}}
\def \AC {{\sf AC}}
\def \BPTIME {{\sf BPTIME}}
\def \SPACE {{\sf SPACE}}
\def \EXP {{\sf EXP}}
\def \EXPSPACE {{\sf EXPSPACE}}
\def \PSPACE {{\sf PSPACE}}
\def \bin {{\sf bin}}
\def \NT {{\sf NTIME}}
\def \NTIME {\NT}
\def \coNT {{\sf coNTIME}}
\def \coNTISP {{\sf coNTISP}}
\def \coNTIME {\coNT}
\def \MOD {{\sf MOD}}
\def \ZPEXP {{\sf ZPEXP}}
\def \ZPTIME {{\sf ZPTIME}}
\def \ZPP {{\sf ZPP}}
\def \V {{\sf V}}
\def \DT {{\sf DTIME}}
\def \DTIME {\DT}
\def \isin {\subseteq}
\def \isnotin {\nsubseteq}
\def \L {{\sf LOGSPACE}}
\def \LOGSPACE {\L}
\def \N {{\mathbb N}}
\def \NEXP {{\sf NEXP}}
\def \SIZE {{\sf SIZE}}
% \def \COMPLEX {\text{{\tt COMPLEX}}}

\DeclareMathOperator*{\tr}{\text{Tr}}

\newcommand{\eq}[1]{Eq.~(\ref{eq:#1})}

\newcommand{\optx}{x^*}
\newcommand{\optd}{d^*}
\newcommand{\xt}[1]{x_{#1}}
\newcommand{\dt}[1]{d_{#1}}
\newcommand{\gt}[1]{g_{#1}}
\newcommand{\nbu}{\cbu \log 1 / \delta}
\newcommand{\nit}{\cgd \log dn}
\newcommand{\rady}{300\lprp{\sqrt{\Tr \Lambda/k} + \beta^{\frac{1}{1 + \alpha}}}}
\newcommand{\rad}{10^6\lprp{\sqrt{\frac{d}{n}} + \lprp{\frac{d}{n}}^{\frac{\alpha}{1 + \alpha}} + \lprp{\frac{\log 1 / \delta}{n}}^{\frac{\alpha}{1 + \alpha}}}}
\newcommand{\radthm}{10^8\lprp{\sqrt{\frac{d}{n}} + \lprp{\frac{d}{n}}^{\frac{\alpha}{1 + \alpha}} + \lprp{\frac{\log 1 / \delta}{n}}^{\frac{\alpha}{1 + \alpha}}}}
\newcommand{\smean}{\tld{\mu}}

\newcommand{\mt}{MT}
\newcommand{\thr}{\tau}
\newcommand{\hth}{\mathcal{HT}}
\newcommand{\med}{Median}
\newcommand{\vthr}{100 n^{\frac{1}{1 + \alpha}}d^{-\frac{(1 - \alpha)}{2(1 + \alpha)}}}
\newcommand{\dd}{\Delta}

\newcommand{\radAlg}{20\radst}
\newcommand{\radAlgG}{25\radst}
\newcommand{\radRet}{30\radst}
\newcommand{\radst}{r^*}

\newcommand{\proj}{\mathcal{P}}
\newcommand{\projp}{\mathcal{P}^\perp}

\newcommand{\mbf}[1]{\mathbf{#1}}
\newcommand{\tld}[1]{\widetilde{#1}}
\newcommand{\ts}{\thicksim}
\newcommand{\normtto}[1]{\norm{#1}_{2 \to 1}}
\newcommand{\ns}{\mc{N}}

\newcommand{\rob}{\eta}
\newcommand{\rate}{\sqrt{\frac{d}{n}} + \lprp{\frac{d}{n}}^{\alpha / (1 + \alpha)} + \lprp{\frac{\log 1 / \delta}{n}}^{\alpha / (1 + \alpha)}}

\newcommand{\cgd}{10^6}
\newcommand{\cbu}{4000}
